SyncViolinist: Music-Oriented Violin Motion Generation Based on Bowing and Fingering

Automatically generating realistic musical performance motion can greatly enhance digital media production, often involving collaboration between professionals and musicians. However, capturing the intricate body, hand, and finger movements required for accurate musical performances is challenging. Existing methods often fall short due to the complex mapping between audio and motion, typically requiring additional inputs like scores or MIDI data. In this work, we present SyncViolinist, a multi-stage end-to-end framework that generates synchronized violin performance motion solely from audio input. Our method overcomes the challenge of capturing both global and fine-grained performance features through two key modules: a bowing/fingering module and a motion generation module. The bowing/fingering module extracts detailed playing information from the audio, which the motion generation module uses to create precise, coordinated body motions reflecting the temporal granularity and nature of the violin performance. We demonstrate the effectiveness of SyncViolinist with significantly improved qualitative and quantitative results from unseen violin performance audio, outperforming state-of-the-art methods. Extensive subjective evaluations involving professional violinists further validate our approach. The code and dataset are available at https://github.com/Kakanat/SyncViolinist.

==> docs/00_abstract/abstract.tex <==
This paper describes a deep-learning-based method for motion generation
    for violin performance.
With the recent development of deep generative models,
    music-oriented body movement generation has been achieved 
    by predicting joint positions or rotations from audio features. 
However,
    it is still challenging to estimate adequate movements 
    due to the complex relationship between audio and body movements.
To address this challenge,
    we propose SyncViolinst,
    a multi-stage, end-to-end framework
    to generate violin performance motion
    from audio input alone.
This approach overcomes the challenge of
    establishing a global-fine correspondence for natural motion generation 
    with a \textit{bowing/fingering model} and \textit{motion generation model}.
Specifically, 
    the bowing/fingering model extracts information
    including bow direction, played string, finger number, and position
    from audio features.
Then, 
    the motion generation model outputs body movements
    using this bowing/fingering information 
    as well as audio features.
To support this method,  
    we also built a dataset
    that includes fine-recorded motion capture data, 
    including finger movements, 
    along with corresponding audio and well-annotated bowing/fingering information,
    which will be published for the future research community. 
We demonstrate 
    that the proposed method is capable of generating more natural and accurate movements
    from unseen violin performance audio
    through extensive evaluations,
    including subjective evaluation involving professional violinists.

==> docs/00_abstract/abstract_ver2.tex <==
Automatically generating natural and realistic musical performance motion has the
potential to significantly enhance digital media production workflow, which often
involves collaboration between professionals and musicians. However, musical
performance motion is challenging and complex as it requires natural global body
movements to convey expressiveness and dictate the rhythm, alongside precise and fine-grained hand and finger movements to perform the correct notes. Current
approaches often fail to capture such global-fine features present in musical
performance due to the ambiguous mapping between audio and body movements, and
typically require additional input such as score or MIDI information to achieve high-quality results. 
In this work, we focus on violin performance and propose
SyncViolinist, a multi-stage, end-to-end framework designed to generate synchronized violin performance motion only from audio input. Our method addresses the challenge of capturing both global and fine-grained features of musical performance by employing a bowing/fingering model and a motion generation model. Recognizing that performers often integrate their interpretation of bowing and fingering into their body movements, our approach leverages this nature to provide useful cues for plausible motion. 
Specifically, the bowing/fingering model extracts fine-grained information about bowing and fingering from audio input, which is then used by the motion generation model to generate refined and and coordinated global movements that consider temporal granularity and motion natures. 
We demonstrate the capability of the proposed method with significantly improved qualitative and quantitative results from unseen violin performance audio compared to state-of-the-art methods. We further validate our method through an extensive subjective evaluation with professional violinists. 
To contribute to future research, we plan to release the captured dataset used in this work, which includes accurately annotated bowing/fingering information, body movements, and synchronized audio. 

==> docs/00_abstract/abstract_ver3.tex <==
% Automatically generating natural and realistic musical performance motion has the potential to significantly enhance digital media production workflows, which often involve collaboration between professionals and musicians. However, musical performance motion is challenging and complex, as it requires natural global body movements to convey expressiveness and dictate rhythm, alongside precise, fine-grained hand and finger movements to perform the correct notes. Current approaches often fail to capture these global-fine features due to the ambiguous mapping between audio and body movements, and typically require additional input such as scores or MIDI information to achieve high-quality results.
% %
% In this work, we focus on violin performance and propose SyncViolinist, a multi-stage, end-to-end framework designed to generate synchronized violin performance motion solely from audio input. Our method addresses the challenge of capturing both global and fine-grained features of musical performance by employing a bowing/fingering module and a motion generation module. Recognizing that performers often integrate their interpretation of bowing and fingering into their body movements, our approach leverages this nature to provide useful cues for plausible motion.
% %
% Specifically, the bowing/fingering module extracts fine-grained information about bowing and fingering from the audio input, which is then used by the motion generation module to generate refined and coordinated global motion \textcolor{blue}{for different body semantics based on the temporal granularity and nature of the violin performance.}
% %
% We demonstrate the capability of the proposed method with significantly improved qualitative and quantitative results from unseen violin performance audio compared to state-of-the-art methods. We further validate our method through an extensive subjective evaluation with professional violinists.
% %
% To contribute to future research, we plan to release the captured dataset used in this work, which includes accurately annotated bowing/fingering information, body motions, and synchronized audio. \textcolor{blue}{The project can be accessed from \url{https://anonymous.4open.science/r/sync-violinist-anon/} (anonymized for submission)}.


\textcolor{blue}{
Automatically generating natural and realistic musical performance motion has the potential to significantly enhance digital media production, which often involves collaboration between professionals and musicians. However, musical performance motion is complex, requiring expressive global body movements and precise hand and finger motions to play correct notes. Current methods often fail to capture these intricate features due to the ambiguous mapping between audio and body motions, and typically need additional inputs like scores or MIDI data to achieve high-quality results.
In this work, we focus on violin performance and propose SyncViolinist, a multi-stage, end-to-end framework designed to generate synchronized violin performance motion solely from audio input. Our method addresses the challenge of capturing global and fine-grained performance features using a bowing/fingering module and a motion generation module. Recognizing that performers integrate their interpretation of bowing and fingering into their body movements, our approach leverages these natural cues to produce plausible motion.
The bowing/fingering module extracts detailed bowing and fingering information from the audio input, which the motion generation module then uses to create refined and coordinated global motion, adapting to the temporal granularity and nature of the violin performance.
We demonstrate the capability of our method with significantly improved qualitative and quantitative results from unseen violin performance audio, compared to state-of-the-art methods. Our approach is further validated through extensive subjective evaluation with professional violinists.
To support future research, we plan to release the code and dataset used in this work, which includes accurately annotated bowing/fingering, body motions, and synchronized audio. The project can be accessed at \url{https://anonymous.4open.science/r/sync-violinist-anon/} (anonymized for submission)}.


==> docs/01_introduction/01_introduction_ver3.tex <==
% (1) First paragraph: the big background. Feel free to discuss or leave comments.
The generation of realistic and natural character movements is crucial to modern digital media production and virtual reality experiences. To achieve a high level of realism, traditional methods are often costly and labor-intensive, involving specialized techniques such as hand-crafting animations and time-consuming motion capture processes. This is particularly true for musical performances, where the consultation of specialized artists is often necessary during the hand-crafting or post-processing stages, disrupting the production flow and impeding the creative process.

% (2) Rewritten second paragraph: Major challenges -> The background of the problem we are trying to solve.
A framework that allows the automatic generation of natural and realistic motion in musical performance from only audio has the potential to significantly improve workflow efficiency and is highly desirable. 
This paper focuses on violin performance and aims to generate body movements from audio signals.
In violin performance, 
the primary hand movements that affect the sound produced on the instrument are 
\textit{bowing} and \textit{fingering}. 
Bowing, which is executed by the right hand, involves the movement of the bow across the strings, whereas fingering, which is performed by the left hand, involves pressing the strings on the frets to control pitch. The performer's interpretation of the musical piece is reflected in the sounds and corresponding body movements through bowing and fingering.

% (3) Existing work, how they tried to deal with the challenges but why they cannot fully solve the challenge.
Creating an automatic system, however, is a challenging task as it requires capturing both natural global body movements to catch the rhythm and precise fine-grained hand and finger movements to play the correct scales. Previous rule-based~\cite{Yin:05} and data-driven~\cite{Serafin:01, Zhu:13, Yamamoto:10} approaches often require additional inputs, such as corresponding musical scores and MIDI information, which limits their practicality. While learning-based methods have demonstrated success in establishing the complex correspondence between motion and audio in an end-to-end manner~\cite{Shlizerman:18, Kao:20, Chen:21}, they often fail to capture the fine features present in musical performance. This is partially due to the numerous correspondences between sound and body movements, leading to the generation of averaged movements.

% (4) Our method overview, how this can deal with the challenge (i.e. better than existing work) -> this will be our contribution (start with “In this paper, we propose a … for …”, if possible give a statement about the hypothesis (e.g. We believe that the characteristics of MWEs are dramatically different from single words), give an overview of the method for the sake of motivating the contributions, highlight the contributions.
In this paper, we propose SyncViolinist, a multi-stage end-to-end framework to generate synchronized violin performance motion from audio input only. This approach overcomes the challenge of establishing a global-fine correspondence for natural motion generation through a \textit{bowing/fingering model} and \textit{motion generation model}.
%Considering that the number of combinations of fingering and bowing can be limited when given tone and pitch, we first propose a convolutional recurrent neural network (CRNN) that predicts the bowing and fingering from the Mel-scaled spectrogram extracted from the input audio.
As mentioned above, performers convey their interpretation of the musical piece not only by the global body movements but by the fine-grained bowing and fingering information.
Based on this fact, we adopt a convolutional recurrent neural network (CRNN) that predicts the bowing and fingering from the Mel-scaled spectrogram extracted from the input audio to incorporate the fine-grained information into the estimation.
Furthermore, we propose a novel model based on the bidirectional long short-term memory (BiLSTM) network that considers both audio features, such as volume and rhythm, and fine-grained features provided by the CRNN to predict the global-fine motion of the violin performance.
Due to the fine-grained information passed to the motion generation model, we narrow down the infinite patterns of global body movements to a limited number of combinations.
To facilitate the integrated learning of audio, body movements, and bowing/fingering, we present a new dataset of synchronized motion and audio signals with accurately annotated bowing/fingering information. We plan to make the dataset publicly available for future research.
% As performers often incorporate their interpretation of the piece (bowing and fingering) into their body movements in real-world performances, we narrow down the infinite patterns of global body movements by passing the fine-grained information to the motion generation model. 
% We propose a novel model based on bidirectional long short-term memory (BiLSTM) that takes into account both audio features, such as volume and rhythm, and fine-grained features provided by the CRNN to predict the global-fine motion of the violin performance. 


% (5) An overview of experimental results, how they support the contributions, where is the application domain.
The experimental results of this study demonstrate that the proposed approach can accurately estimate a time series of joint positions from acoustic features when compared to state-of-the-art methods. In addition, an ablation study was conducted to further demonstrate the effectiveness of incorporating bowing/fingering information. Furthermore, an extensive subjective evaluation involving 17 professional violinists was conducted, which revealed that the generated motion possessed a higher level of realism.

% (6) conclusion
The contribution of this work is two-fold;
\begin{itemize}
    \item we propose a novel multi-stage, end-to-end framework that generates realistic and natural motion for violin performance from audio signals via bowing/fingering information;
    \item we construct an entirely new dataset 
    of professional players
    with synchronized bowing/fingering information, audio signals, and body movements, which will be released for the future research community. 
\end{itemize}


==> docs/04_dataset/04_1.tex <==
% To capture motion data,
%     we utilize a motion capture system,
%     which is based on 16 synchronized cameras recording motion at 120 fps.
% The performer wore Vicon's suits with 57 optical markers
%     and had 20 markers attached to their fingers.
% The resulting data included the 3-D positions of each marker over time,
%     providing a detailed representation of the violinist's finger
%     and body movements during the performance.    
% We simultaneously recorded audio and MIDI data using a violin
%     that can output audio and MIDI signals at the same time
%     during motion capture.   
% The audio signals were recorded on line output at a sampling rate of 44.1 kHz,
%     taking care to exclude any room noise.
% The MIDI data was also recorded for use in the post-processing stage.
% It should be noted that
%     while the MIDI signals were used to aid in the annotation of the data, 
%     they will not be used as the input of our model.

% To acquire motion data, we employed a motion capture system that utilizes 16 synchronized cameras operating at 120 fps. The performer wore a suit with 57 optical markers provided by Vicon, and an additional 20 markers were attached to the fingers. This resulted in the collection of the 3D positions of each marker over time, providing a detailed representation of the violinist's finger and body motions during the performance. Additionally, we simultaneously recorded audio and MIDI data using a violin that can output both audio and MIDI signals during motion capture. The audio signals were recorded on line output at a sampling rate of 44.1 kHz, with care taken to eliminate any room noise. The MIDI data was also recorded for use in the post-processing stage. It is worth noting that while the MIDI signals were used to aid in the annotation of the data, they will not be used as input to our model.

% In addition to the motion and audio data,
%     we collected well-annotated fingering and bowing information for each performance. 
% The performers themselves entered this information into the music score data
%     (in MusicXML format) beforehand, 
%     specifying the bow up/down and finger number for each note.
% Altogether, 
%     we collected 182 minutes of performance data (54 songs) from three violinists.

% Along with the motion and audio data, we obtained well-annotated information on fingering and bowing techniques for each performance. The performers themselves entered this information into the music score data (in MusicXML format) prior to the recording, indicating the bow up/down and finger number for each note. 
% % In total, we collected 182 minutes of performance data (54 songs) from three violinists.
% \textcolor{blue}{In total, we collected ?? minutes of performance data, 61 pieces, from 3 violinists.}


==> docs/04_dataset/04_2.tex <==
% To meet the need of our model training task,
%     we post-processed the recorded motion, audio, and bowing/fingering information.
    
% First, 
%     the motion data is post-processed with Shugon, a motion editing software, 
%     resulting in the rotation information in Euler angles of 61 joints 
%     and the 3d positions of the root
%     (24 for the body and 38 for the fingers).
% Then, 
%     we downsampled the motion data to 30 fps
%     and calculated the 3-D joint position $Y\in \mathbb{R}^{62 \times 3 \times T}$
%     from the rotation representation on the basis of forward kinematics,
%     where $T$ indicates the number of time frames.
% We also retargeted the motion data to a common skeleton
%     to eliminate the effect of differences in the violinists' body sizes and shapes, 
%     but not to change their hand and fingertip positions.
% Finally, 
%     the motion data was normalized 
%     to ensure 
%     that the temporal mean of all joints is zero and the variance is one.

% To prepare the data for training our model, we performed post-processing on the recorded motion, audio, and bowing/fingering information, and the final outputs include: bow direction $L^{\mathrm{bow}}$, played string $L^{\mathrm{str}}$, finger number $L^{\mathrm{fing}}$, and position sequence $L^{\mathrm{pos}}$.}

% Moved this section to the supplementary material

First, we used Shugon, a motion editing software, to process the motion data and obtain the rotation information in Euler angles for \textcolor{blue}{??} joints and the 3D positions of the root (24 for the body and 38 for the fingers). Next, we downsampled the motion data to 30 fps and calculated the 3D joint position $Y\in \mathbb{R}^{T \times 62 \times 3}$ from the rotation representation using forward kinematics, where $T$ represents the number of time frames. Additionally, we retargeted the motion data to a common skeleton to eliminate the effect of variations in the violinists' body sizes and shapes, while keeping their hand and fingertip positions intact. 

To extract audio features from the recorded signals, we used librosa, a Python library for music signal processing ~\cite{Mcfee:15}. We applied a short-time Fourier transform (STFT) with a sliding window of length 2048 samples and a hop size of 1/30 seconds to obtain a 128D Mel spectrogram $X\in \mathbb{R}^{T \times 128}$. 

To obtain the fingering and bowing information that is synchronized with the motion data, we used both the recorded MIDI signals and the MusicXML scores that were annotated by the violinists. It is worth noting that the MIDI signals were recorded simultaneously with the audio signals, thus by annotating each label of the bowing/fingering information for each MIDI note, synchronization of audio features and bowing/fingering information can also be guaranteed at the same time. Since the bow direction and finger number labels were annotated in MusicXML by the violinists themselves, we were able to correspond the bow direction and finger number labels for each MIDI note actually played by synchronizing the MusicXML with the MIDI signals using a MIDI-to-score alignment method~\cite{Nakamura:17}.    
However, since this alignment is sometimes inaccurate, we manually corrected the information. For string labels, we have obtained them by identifying which of the four channels had the largest output at each time frame, since the MIDI violin used in our dataset acquisition process had outputs from different channels for each of the four strings.
As for position labels, we decided them from the recorded MIDI note number (\textit{i.e.} pitch), played string and the finger number obtained above.

\textcolor{blue}{After annotating each label in bowing/fingering information to the MIDI notes, we finally converted them to ensure that they were consistent with the time frame of audio features. The final outputs include: bow direction $L^{\mathrm{bow}}$, played string $L^{\mathrm{str}}$, finger number $L^{\mathrm{fing}}$, and position sequence $L^{\mathrm{pos}}$.}

==> docs/05_evaluation/05_3.tex <==
% We employed three methods as the baseline
%     that generates musical instrument performance motion 
%     from audio signals similar to our method.
% The baselines include
%     LSTM-based method ~\cite{Shlizerman:18},
%     two-branch network-based method ~\cite{Kao:20},
%     and GAN-based method~\cite{Chen:21}.
% While the first two of them output joint positions similar to ours,  
%     the last one output joint rotations.
% % Thus,
% %     in quantitative evaluation,
% %     we calculate the joint position on the basis of forward kinematics
% %     as for the output by ~\cite{Chen:21}.
% Therefore, in the quantitative evaluation, we calculated the joint position on the basis of forward kinematics for the output of ~\cite{Chen:21} for a fair comparison.

% \subsubsection{Quantitative results}
% \autoref{table:quant_comparison} shows the quantitative results.
% \{L1, DTW\} indicate the measure for all joints,
%     \{L1RH, DTWRH\} indicate the measure for the right arm,
%     \{L1LH, DTWLH\} indicate the measure for the left arm,
%     and \{L1LF, DTWLF\} indicate the measure for the fingers of the left hand.
% Each score represents the average of the entire test set.
% As shown in the table,
%     our method outperforms all the baseline methods in all scores.
% The results indicate
%     that our method is effective in generating more accurate body motions
%     with accurate sequences
%     in comparison with all the baseline methods,
%     including hand-related motions.

\subsubsection{Subjective evaluation results}
\label{subsubsec:sub_comparison}
% \autoref{fig:sub_comparison} shows the average scores
%     and standard deviations of the ratings
%     obtained by all the methods and the ground truth,
%     and the p-value of the Mann-Whitney U test
%     done on the minimal distance (** indicates the 0.001 level of significance)
%     between the proposed methods and others.    
% We show the results separately
%     for those with and without violin-playing experience.
% The results show that our method can outperform all the baseline methods 
%     in terms of naturalness
%     for both experienced and inexperienced participants,
%     while others are not in this experiment.
% \autoref{fig:sub_comparison} presents the average scores and the standard deviations of the ratings. The results are presented separately for participants with and without violin-playing experience. 
% To statistically analyze the obtained data,
%     we also performed paired Mann-Whitney U test ~\cite{McKnight:10}.
% The results are shown in \autoref{table:sub_comparison}, where * indicates the 0.01 significance.
% The results demonstrate that our method outperforms all the baseline methods in terms of naturalness for both experienced and inexperienced participants, although experienced participants tended to have a larger difference between the scores for the ground truth and for the generated results.
% %while the other methods do not achieve this in this experiment.
% On the other hand, 
%     our method is still significantly inferior to the ground-truth motion data.
% This indicates that 
%     there is still room for improvement in our method.
% Please refer to the supplementary material for more detailed examples of the animation.

% %, and p-value of the Mann-Whitney U test for the minimal distance (** indicates 0.001 level of significance) between the proposed method and other methods.

==> docs/old_version/01_introduction.tex <==
% target topic and its importance
Creating characters that behave naturally like humans is a key component     
    in providing viewers with a realistic experience 
    in computer-animated movies or VR.
This is also true for animations  
    where characters play musical instruments synchronized to music.
However, 
    a significant challenge here is 
    that musical instrument performance requires fine-grained body movements to produce the intended sound, 
    which makes it difficult to reproduce such animations.

% standard and previous approaches 
One solution to the problem is the usage of motion capture tools. 
While these tools enable us to capture accurate body movements,
    the usage of these tools has the drawbacks 
    of requiring recording with an actor every time, 
    specialized skills, 
    and laborious post-processing.
Another approach to solve this problem 
    is to automatically generate musical performance animations
    on a basis of novel inputted music without human intervention.
Recent developments in machine learning, 
    especially deep learning, 
    have led to the emergence of methods 
    for automatic generation of body movements for musical performance 
    from an input of music, either acoustic features or musical scores.
%(もっと具体的な例を追加する)
Although these methods have made it possible
    to generate musical performance movements in an end-to-end manner, 
    it is still challenging to generate fine-grained movements.
This is partly due to the innumerable correspondences
    between sound and body movements, 
    resulting in "smoothing" of the generated movements.

% our solution
Body movements during a musical performance would be considered
    to be transformed from performers' conceptual interpretation 
    of the musical structures and units~\cite{Palmer:97}.
In violin performances,
    there are mainly two parts of movements that reflect their intention; 
    \textit{fingering} and \textit{bowing}.
Fingering is a movement carried by the left hand 
    to control the pitch by pressing the strings on the frets.
Mostly, an identical note can be played on different strings with different fingers and position.
Since music scores do not usually indicate which fingers to play with for every note 
    but only for several important notes.
Thus, 
    the whole fingering is dependent on what kind of tone the performer intends to produce
    as every string has its specific tone~\cite{Galamian:13}.
Similarly, 
    the right hand executes bowing to make the bow move across the string.
Typically,
    there are two bowing modes: up-bow and down-bow.
Since the score generally indicates bowing instruction for several notes, as well as fingering, 
    most bowing is dependent on how the performer segments the notes.
Thus, 
    the performer determines the fingering and bowing according to their interpretation at first, 
    and these decisions are reflected in the tones and their body movements.
%The left hand carries the fingering,
%    which is decided in order to assure the best sound and finest expression of the phrase and to make the passage as easy and comfortable as possible~\cite{Galamian:13}.
%In contrast, 
%    the right hand carries the bowing,
%    which is decided  

%Technical details
In this paper, 
    we propose SyncViolinist,
    a novel method for audio-to-body movements synthesis for violin performance
    drawing on the nature of how body movements are generated during a musical performance.
Following ~\cite{Hirata:22},
    we first estimate hand-related playing procedure information,
    which contains string, finger, position, and bow direction.
Then,
    we build the body movement generative model taking them as input in addition to audio features.
In this part, 
    we adopt a curriculum learning method
    to make the output movements finer.
Moreover,
    to investigate the mapping between audio features and the body movements mediated by the playing procedure information,
    we propose a new dataset that contains playing procedure information along with the corresponding audio signals and performers' body movements.

% conclusion
The contributions of this paper are thus;

\begin{itemize}
    \item we develop a cross-domain embedding framework, incorporating the playing procedure information to correctly generate the body movements for violin performance;
    \item we develop a new dataset to investigate the mapping between playing procedure information, audio signals, and body movements;
    \item we investigate whether our model can generate fine body movements to input audio through evaluation.  
\end{itemize}

    
    

==> docs/old_version/01_introduction_ver2.tex <==
% target topic
% Creating characters with natural and realistic movements 
%     is crucial in movie and VR production,     
%     as it helps to immerse viewers in the experience. 
% However, 
%     generating such motions requires costly processes such as hand-crafting and motion capture. 
% The traditional method of handcrafting animations is labor-intensive
%     and requires specialized skill. 
% Also,
%     while motion capture systems can capture realistic movements, 
%     they still require actors every time
%     and can be difficult to use for a large number of patterns.
% Additionally, 
%     post-processing the captured motion requires specialized knowledge 
%     and can take a significant amount of time. 
% To overcome these challenges, 
%     there is a growing demand for automation in motion generation.
% As one of the main approaches to this,
%     researchers have been exploring ways to generate body movements from audio signals,
%     such as creating body movements of musicians from audio, 
%     generating facial expressions and hand gestures from conversational speech, 
%     and generating choreographic movements from music.

% Rewritten first paragraph; bigger background.
% Creating realistic and natural character movements is essential for immersive movie experiences and virtual reality productions.
% However, achieving a high level of realism is often a costly and labor-intensive process, involving techniques such as hand-crafting animations and motion capture. 
% The traditional method of hand-crafting animations requires specialized skills and is time-consuming. 
% Additionally, while motion capture systems can capture realistic movements, they still require actors and can be difficult to use for a large number of patterns. 
% Post-processing the captured motion also requires specialized knowledge and can take a significant amount of time. 
% To address these challenges, there is a growing demand for automation in motion generation. 
% Researchers have been exploring various approaches, such as creating body movements of musicians from audio, producing facial expressions and hand gestures from conversational speech, and generating choreographic movements from music.

% motion generation for violin performance
% In this paper, 
%     we specifically focus on the task of generating body movements
%     for violin performance.
% Violinists' body movements are complicated
%     due to several reasons.
% Performers typically execute a series of movements 
%     that include subtle movements of the head and body to convey expressiveness, 
%     movement of the torso to dominate the rhythm,
%     and precise hand movements to play accurate notes with intended sounds.
% As for violin performance,
%     there are mainly two parts of hand movements 
%     that affect the sounds produced by the violin; 
%     \textit{bowing} and \textit{fingering}.
% Bowing is a series of movements carried by the right hand 
%     to make the bow move across the string.
% Typically,
%     there are two bowing modes: up-bow and down-bow.
% Since the music score 
%     generally indicates bowing instruction for several important notes, 
%     most bowing is dependent on how the performer segments the notes.
% Similarly,
%     the left hand executes fingering  
%     to control the pitch by pressing the strings on the frets.
% Mostly, 
%     an identical note can be played on different strings
%     with different fingers and positions.
% As the same as bowing instruction,
%     music scores do not usually indicate which fingers to play with
%     for every note but only for several important notes.
% Thus, 
%     the whole fingering is dependent on what kind of tone the performer intends to produce
%     as every string has its specific tone~\cite{Galamian:13}.
% Thus, 
%     the performer determines the fingering and bowing according to their interpretation at first, 
%     and these decisions are reflected in the sounds and their body movements.

% Rewritten second paragraph; smaller background, and previous methods.
In this paper, we focus on the task of generating body movements for violin performance. 
The movements of violinists are complex as they involve subtle head and body movements to convey expressiveness, movement of the torso to dictate the rhythm, and precise hand movements to play accurate notes. 
In violin performance, the two main hand movements that affect the sounds produced by the violin are \textit{bowing} and \textit{fingering}. 
Bowing, a series of movements carried out by the right hand, involves moving the bow across the string. 
Fingering, executed by the left hand, involves pressing the strings on the frets to control pitch. 
The performer determines the fingering and bowing according to their interpretation~\cite{Galamian:13} and these decisions are reflected in the sounds and their body movements.


%previous methods
To generate musical performance animation beyond violin performance, 
    various attempts have been made.
A variety of methods, 
    including rule-based, data-driven, and learning-based methods,
    have been devised to automate the generation of performance motion.
In recent years, 
    there has been a significant advancement
    in the use of deep neural network-based generative models
    to capture more complex correspondence between audio and body movements. 
They have demonstrated success
    in generating expressive performance motion
    in an end-to-end manner.
% problems of the previous methods 
However, 
    it is still challenging to generate fine-grained movements.
This is partly due to the innumerable correspondences
    between sound and body movements, 
    resulting in "smoothing" of the generated movements.

% our solution
In this paper, 
    we propose SyncViolinist,
    a novel approach to motion generation 
    for violinists to \textit{synchronize} with the input audio,
    coming back to the nature of how violinists' body movements occur.
As mentioned above, 
    performers play the violin 
    after symbolically determining the bowing and fingering.
In other words,
    the information about bowing and fingering is transmitted
    in the process of body movements and sounds occur.
In motion generation,
    passing on this fingering and bowing information
    will make it easier to estimate violinists' body movements 
    than generating them directly from audio as well.
First,
    bowing and fingering is easier to estimate from audio.
This is due to the fact that
    the number of combinations of fingering and bowing is limited to a few
    for a given tone and pitch, 
    while infinite patterns of body movements spread over a continuous space.
Then, 
    when the information on fingering and bowing is provided
    during motion generation, 
    the space of predicted body movements can be narrowed,
    as the fingering and bowing determined by the performer
    are strongly reflected to their motion.
Considering the above,
    we designed our motion generation method
    via bowing and fingering information.
    
%Technical details
In details, 
    we propose a multi-stage framework 
    consisting \textit{bowing/fingering model}
    and \textit{body movements model}.
In the bowing/fingering model, 
    we estimate the time series of four features with convolutional recurrent neural network (CRNN)
    from mel-scaled spectrogram extracted from input audio:
    bow direction, played string, finger number, and position,
In the body movements model,
    we build a model based on bidirectional long short-term memory (BiLSTM) 
    that takes as inputs both audio features and the four features estimated in the previous bowing/fingering model
    and outputs the time series of joint positions of a violinist. 
This allows us to consider 
    both time series of bowing/fingering information
    that explicitly related to body movements 
    and other features such as volume and rhythm, 
    which are included in the audio features 
    but not in the bowing/fingering information alone.
To further investigate the relationship
    between audio, body movements, and bowing/fingering, 
    we have constructed a new dataset 
    that includes simultaneously recorded motion and audio signals,
    and well-annotated bowing/fingering.
For the motion data, 
    we used a VICON motion capture system
    to accurately measure body movements including finger 
    and recorded them along with audio of violin performances. 
In addition, 
    to obtain accurate information on fingering/bowing,
    we asked the performers to annotate it 
    and synchronized it with the audio information
    using a method that aligns the score and performance.
We plan to make this dataset publicly available for future research.

% conclusion
The contributions of this paper are thus;

\begin{itemize}
    \item we propose a multi-stage framework
    via bowing/fingering information 
    to correctly generate body movements for violin performance
    from audio signals;
    \item we constructed a new dataset
    to investigate the mapping 
    between bowing/fingering information, audio signals, and body movements,
    which will be released for the future research community. 
\end{itemize}
Finally, 
    we demonstrate
    that our model is capable of generating fine body movements
    for violin performance
    from the input audio 
    through extensive evaluations.
We also show the effectiveness 
    of the four components of bowing/fingering information 
    through an ablation study.
    

==> figs_and_tables/joint_list1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\begin{tabular}{clccc}
\toprule
\multirow{2}{*}{Node number} & \multirow{2}{*}{Joint name} & \multirow{2}{*}{Parent node} & \multicolumn{2}{c}{Body parts}   \\
\cmidrule(lr){4-5}
    &   &   & in generation & in evaluation    \\ 
\midrule
0                            & Hips                        & -                            & Others        & -                \\
1                            & Spine                       & 0                            & Others        & -                \\
2                            & Spine1                      & 1                            & Others        & -                \\
3                            & Spine2                      & 2                            & Others        & -                \\
4                            & Spine3                      & 3                            & Others        & -                \\
5                            & Neck                        & 4                            & Others        & -                \\
6                            & Neck1                       & 5                            & Others        & -                \\
7                            & Head                        & 6                            & Others        & -                \\
8                            & End Site                         & 7                            & Others        & -                \\
9                            & RightShoulder               & 4                            & Others        & -                \\
10                           & RightArm                    & 9                            & Others    & -                \\
11                           & RightForeArm                & 10                           & Right hand    & Right arm (RA)    \\
12                           & RightHand                   & 11                           & Right hand    & Right arm (RA)    \\
13                           & RightHandMiddle1            & 12                           & Right hand    & -                \\
14                           & RightHandMiddle2            & 13                           & Right hand    & -                \\
15                           & RightHandMiddle3            & 14                           & Right hand    & -                \\
16                           & End Site                         & 15                           & Right hand    & -                \\
17                           & RightHandRing               & 12                           & Right hand    & -                \\
18                           & RightHandRing1              & 17                           & Right hand    & -                \\
19                           & RightHandRing2              & 18                           & Right hand    & -                \\
20                           & RightHandRing3              & 19                           & Right hand    & -                \\
21                           & End Site                         & 20                           & Right hand    & -                \\
22                           & RightHandPinky              & 17                           & Right hand    & -                \\
23                           & RightHandPinky1             & 22                           & Right hand    & -                \\
24                           & RightHandPinky2             & 23                           & Right hand    & -                \\
25                           & RightHandPinky3             & 24                           & Right hand    & -                \\
26                           & End Site                    & 25                           & Right hand    & -                \\
27                           & RightHandIndex              & 12                           & Right hand    & -                \\
28                           & RightHandIndex1             & 27                           & Right hand    & -                \\
29                           & RightHandIndex2             & 28                           & Right hand    & -                \\
30                           & RightHandIndex3             & 29                           & Right hand    & -                \\
31                           & End Site                         & 30                           & Right hand    & -                \\
32                           & RightHandThumb1             & 27                           & Right hand    & -                \\
33                           & RightHandThumb2             & 32                           & Right hand    & -                \\
34                           & RightHandThumb3             & 33                           & Right hand    & -                \\
35                           & End Site                         & 34                           & Right hand    & -                \\
\bottomrule         
\end{tabular}
 \caption{Detailed list of the captured joints from the proposed dataset (1/2).}
 \label{table:joint_list1}
\end{table*}


==> figs_and_tables/joint_list2.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{clccc}
\toprule
\multirow{2}{*}{Node number} & \multirow{2}{*}{Joint name} & \multirow{2}{*}{Parent node} & \multicolumn{2}{c}{Body parts}   \\
\cmidrule(lr){4-5}
    &   &   & in generation & in evaluation    \\ 
\midrule
36                           & LeftShoulder                & 4                            & Others        & -                \\
37                           & LeftArm                     & 36                           & Others      & -                \\
38                           & LeftForeArm                 & 37                           & Left arm      & Left arm (LA)     \\
39                           & LeftHand                    & 38                           & Left arm      & Left arm (LA)     \\
40                           & LeftHandMiddle1             & 39                           & Left hand     & -                \\
41                           & LeftHandMiddle2             & 40                           & Left hand     & -                \\
42                           & LeftHandMiddle3             & 41                           & Left hand     & -                \\
43                           & End Site                         & 42                           & Left hand     & Left fingers (LF) \\
44                           & LeftHandRing                & 39                           & Left hand     & -                \\
45                           & LeftHandRing1               & 44                           & Left hand     & -                \\
46                           & LeftHandRing2               & 45                           & Left hand     & -                \\
47                           & LeftHandRing3               & 46                           & Left hand     & -                \\
48                           & End Site                         & 47                           & Left hand     & Left fingers (LF) \\
49                           & LeftHandPinky               & 44                           & Left hand     & -                \\
50                           & LeftHandPinky1              & 49                           & Left hand     & -                \\
51                           & LeftHandPinky2              & 50                           & Left hand     & -                \\
52                           & LeftHandPinky3              & 51                           & Left hand     & -                \\
53                           & End Site                         & 52                           & Left hand     & Left fingers (LF) \\
54                           & LeftHandIndex               & 39                           & Left hand     & -                \\
55                           & LeftHandIndex1              & 54                           & Left hand     & -                \\
56                           & LeftHandIndex2              & 55                           & Left hand     & -                \\
57                           & LeftHandIndex3              & 56                           & Left hand     & -                \\
58                           & End Site                         & 57                           & Left hand     & Left fingers (LF) \\
59                           & LeftHandThumb1              & 54                           & Left hand     & -                \\
60                           & LeftHandThumb2              & 59                           & Left hand     & -                \\
61                           & LeftHandThumb3              & 60                           & Left hand     & -                \\
62                           & End Site                         & 61                           & Left hand     & Left fingers (LF) \\
63                           & RightUpLeg                  & 0                            & Others        & -                \\
64                           & RightLeg                    & 63                           & Others        & -                \\
65                           & RightFoot                   & 64                           & Others        & -                \\
66                           & RightForeFoot               & 65                           & Others        & -                \\
67                           & RightToeBase                & 66                           & Others        & -                \\
68                           & End Site                         & 67                           & Others        & -                \\
69                           & LeftUpLeg                   & 0                            & Others        & -                \\
70                           & LeftLeg                     & 69                           & Others        & -                \\
71                           & LeftFoot                    & 70                           & Others        & -                \\
72                           & LeftForeFoot                & 71                           & Others        & -                \\
73                           & LeftToeBase                 & 72                           & Others        & -                \\
74                           & End Site                         & 73                           & Others        & -                \\
\bottomrule         
\end{tabular}
 \caption{Detailed list of the captured joints from the proposed dataset (2/2).}
 \label{table:joint_list2}
\end{table*}

==> figs_and_tables/table_cross_violinist.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lcccc}
    \toprule
     Method & L1 & L1RA & L1LA & L1LF\\
     \midrule
      Shlizerman et al.~\cite{Shlizerman:18} & 18.08 & \bf{0.50} & 0.41 & 1.22 \\ %A2BD
Kao and Su~\cite{Kao:20} & 37.50 & 1.93 & 0.44 & 1.30\\ %TGM2B
Chen et al.~\cite{Chen:21} & 20.02 & 0.74 & 0.34 & 1.17\ %TVCG
% \midrule
\bf{Ours} & \bf{17.53} & 0.51 & \bf{0.38} & \bf{1.15}\\
\bottomrule
    \end{tabular}
    \vspace{-1mm}
        \caption{Cross-violinist valildation results.}
        \label{table:cross_violinist}
    \vspace{-4mm}
\end{table*}

==> figs_and_tables/table_sub_ablation.tex <==
\begin{table}[htbp]
    \centering
    \small
    \begin{tabular}{lcc}
    \hline
     & Experienced & Inexperienced  \\
     \hline \hline
w/o $L^{\mathrm{bow}}$ &U=3336.0; p=1.370e-32*	&U=6786.5; p=1.313e-34* \\
w/o $L^{\mathrm{str}}$ &U=12682.5; p=0.885	&U=20436.0; p=0.319\\
w/o $L^{\mathrm{fing}}$ &U=11949.5; p=0.296	&U=20521.0; p=0.356 \\
w/o $L^{\mathrm{pos}}$ &U=12686.5; p=0.889	&U=21291.0; p=0.777\\
\hline
    \end{tabular}
    \caption{Paired Mann-Whitney U test results for the scores by all the models in the ablation study (* indicates the 0.01 levels of significance).}
    \label{table:sub_ablation}
\end{table}

==> figs_and_tables/table_sub_comparison.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{lcc}
    \hline
     & Experienced & Inexperienced  \\
     \hline \hline
      ~\cite{Shlizerman:18} & U=4166.0; p=4.209e-27* & U=8366.5; p=5.135e-28*  \\
~\cite{Kao:20}	& U=6562.0; p=1.226e-14*	& U=14504.5; p=3.618e-09*	 \\
~\cite{Chen:21}	& U=2085.0; p=2.420e-45*	& U=3237.5; p=2.517e-54*	 \\
Ground truth	&U=511.5; p=1.102e-52*	&U=6955.0; p=1.050e-34*\\
\hline
    \end{tabular}
    \caption{Paired Mann-Whitney U test results for the scores by all the baseline and the ground truth (* indicates the 0.01 levels of significance).}
    \label{table:sub_comparison}}

\end{table}
